Missing Modality Robustness in Semi-Supervised Multi-Modal Semantic Segmentation

Using multiple spatial modalities has been proven helpful in improving semantic segmentation performance. However, there are several real-world challenges that have yet to be addressed: (a) improving label efficiency and (b) enhancing robustness in realistic scenarios where modalities are missing at the test time. To address these challenges, we first propose a simple yet efficient multi-modal fusion mechanism Linear Fusion, that performs better than the state-of-the-art multi-modal models even with limited supervision. Second, we propose M3L: Multi-modal Teacher for Masked Modality Learning, a semi-supervised framework that not only improves the multi-modal performance but also makes the model robust to the realistic missing modality scenario using unlabeled data. We create the first benchmark for semi-supervised multi-modal semantic segmentation and also report the robustness to missing modalities. Our proposal shows an absolute improvement of up to 10% on robust mIoU above the most competitive baselines. Our code is available at https://github.com/harshm121/M3L

==> figures/results-lf.tex <==
\begin{figure}
\begin{subfigure}{0.95\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/images/lf-stanford.png}
  \caption{1a}
\end{subfigure}\\
\begin{subfigure}{0.95\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/images/lf-sunrgbd.png}
  \caption{1b}
\end{subfigure}
\caption{plots of....}
\label{fig:fig}
\end{figure}

==> tables/missing-modality-full-sup.tex <==

\begin{table}[h]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{rcccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{Stanford Indoor} & \multicolumn{4}{c}{SUN RGBD} \\
\multicolumn{1}{c}{} & RGB & Depth & RGBD & \multicolumn{1}{l|}{MM-Robust} & RGB & Depth & RGBD & MM-Robust \\ \midrule
Token Fusion & 37.38 & 31.87 & 56.64 & \multicolumn{1}{c|}{41.96} & 42.93 & 36.09 & 47 & 42.01 \\
URN & 29.64 & 34.78 & 55.10 & \multicolumn{1}{c|}{39.84} & 43.44 & 16.87 & 47.99 & 36.1 \\
Linear Fusion & 30.03 & 27.41 & 57.16 & \multicolumn{1}{c|}{38.20} & 43.25 & 20.95 & 48.17 & 37.46 \\
TF + MD & 48.92 & 47.10 & 53.81 & \multicolumn{1}{c|}{49.94} & 44.97 & 37.58 & 45.46 & 42.67 \\
URN + MD & 49.92 & \textbf{50.14} & \textbf{57.25} & \multicolumn{1}{c|}{\textbf{52.84}} & 45.03 & 37.86 & 48.08 & 43.66 \\ \hline
LF + MD & \textbf{51.34} & 49.66 & 56.85 & \multicolumn{1}{c|}{52.62} & \textbf{46.18} & \textbf{38.55} & \textbf{48.22} & \textbf{44.32} \\ \bottomrule
\end{tabular}
}
\caption{Missing Modality in fully supervised training}
\label{tab:missing-modality-full-sup}
\end{table}

==> tables/missing-modality-semi-sup-stanfordindoor.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{%
\begin{tabular}{rllllllllllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{0.1\%  (49)} & \multicolumn{4}{c}{0.2\% (98)} & \multicolumn{4}{c}{1\% (491)} \\
\multicolumn{1}{c}{} & RGB & Depth & RGBD & \multicolumn{1}{l|}{MM-Robust} & RGB & Depth & RGBD & \multicolumn{1}{c|}{MM-Robust} & RGB & Depth & RGBD & MM-Robust \\ \midrule
Uni-modal\cite{segformer} & 35.43 & 34.05 & ~~~- & \multicolumn{1}{l|}{~~~-} & 39.45 & 35.24 & ~~~- & \multicolumn{1}{l|}{~~~-} & 46.45 & 44.78 & ~~~- & ~~~- \\
TF \cite{tokenfusion} & 29.96 & 29.98 & 40.17 & \multicolumn{1}{l|}{33.37} & 33.11 & 31.47 & 43.04 & \multicolumn{1}{l|}{35.87} & 37.34 & 28.33 & 51.85 & 39.17 \\
URN \cite{urn} & 30.56 & 25.85 & 40.17 & \multicolumn{1}{l|}{32.19} & 35.71 & 25.14 & 45.87 & \multicolumn{1}{l|}{35.57} & 36.25 & 33.27 & 52.07 & 40.53 \\
LF & 33.96 & 25.09 & 42.09 & \multicolumn{1}{l|}{33.71} & 33.66 & 24.61 & 46.60 & \multicolumn{1}{l|}{34.96} & 33.51 & 23.70 & 52.47 & 36.56 \\ \midrule
LF + MT~\cite{mt} & 32.37 & 22.92 & 41.77 & \multicolumn{1}{l|}{32.35} & 33.99 & 23.34 & \underline{48.54} & \multicolumn{1}{l|}{35.29} & 33.65 & 22.42 & 54.32 & 36.80 \\
Ours & \textbf{40.05} \add{7.68}& \textbf{39.93} \add{9.95} & \textbf{44.10} \add{2.01} & \multicolumn{1}{l|}{\textbf{41.36} \add{7.65}} & \textbf{44.62} \add{8.91} & \textbf{42.70} \add{11.23}& \textbf{49.05} \add{0.51} & \multicolumn{1}{l|}{\textbf{45.46} \add{9.59}} & \textbf{49.28} \add{11.94} & \textbf{46.79}\add{13.52} & \textbf{55.48} \add{1.16}& \textbf{50.52} \add{9.99}\\\bottomrule
\end{tabular}
}
\caption{Missing Modality robustness on Stanford Indoor \cite{stanfordindoor} for varying amounts of labeled data (49, 98, 491 data points).}
\label{tab:missing-modality-semi-sup-stanford-indoor}
\end{table*}

==> tables/missing-modality-semi-sup-sunrgbd.tex <==
\begin{table*}[ht]
\resizebox{\linewidth}{!}{%
\begin{tabular}{rllllllllllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{6.25\%  (297)} & \multicolumn{4}{c}{12.5\% (594)} & \multicolumn{4}{c}{25\% (1189)} \\
\multicolumn{1}{c}{} & RGB & Depth & RGBD & \multicolumn{1}{l|}{MM-Robust} & RGB & Depth & RGBD & \multicolumn{1}{c|}{MM-Robust} & RGB & Depth & RGBD & MM-Robust \\ \midrule
Uni-modal\cite{segformer} & 28.71 & 22.81 & ~~~- & \multicolumn{1}{l|}{~~~-} & 35.33 & 27.6 & ~~~- & \multicolumn{1}{l|}{~~~-} & 38.31 & 30.43 & ~~~- & ~~~- \\
TF \cite{tokenfusion} & 27.97 & 23.58 & 29.31 & \multicolumn{1}{l|}{26.95} & 33.75 & 28.31 & 35.88 & \multicolumn{1}{l|}{32.65} & 37.36 & 31.90 & 39.86 & 36.37 \\
URN \cite{urn}& 28.72 & 12.47 & \underline{31.31} & \multicolumn{1}{l|}{24.17} & 33.66 & 15.62 & 37.62 & \multicolumn{1}{l|}{28.97} & 37.49 & 17.27 & 40.49 & 31.75 \\
LF & \underline{29.69} & 15.75 & \textbf{32.00} & \multicolumn{1}{l|}{25.81} & 35.48 & 17.46 & \underline{39.00} & \multicolumn{1}{l|}{30.65} & 39.15 & 17.66 & \underline{42.09} & 32.97 \\ \midrule
LF + MT~\cite{mt} & \underline{29.57} & 17.86 & 31.11 & \multicolumn{1}{l|}{26.18} & 34.82 & 18.89 & \underline{39.17} & \multicolumn{1}{l|}{30.96} & 38.96 & 21.03 & \underline{41.95} & 33.98 \\ 
Ours & \textbf{29.92} \add{0.23} & \textbf{25.44} \add{1.86} & 30.67 \sub{1.33} & \multicolumn{1}{l|}{\textbf{28.68} \add{1.73}} & \textbf{38.12} \add{2.64}& \textbf{32.29} \add{4.08} & \textbf{39.70} \add{0.53} & \multicolumn{1}{l|}{\textbf{36.70} \add{4.05}} & \textbf{41.31} \add{2.16} & \textbf{34.11} \add{2.21}& \textbf{42.69} \add{0.6} & \textbf{39.37} \add{3.00}\\ \bottomrule
\end{tabular}
}
\caption{Missing Modality robustness on SUN RGBD \cite{sunrgbd} for varying amounts of labeled data (297, 584, 1189 data points).}
% \yc{Any potential reason why our method perform worse in the case of 6.25\% RGBD? }}
\label{tab:missing-modality-semi-sup-sunrgbd}
\end{table*}

==> tables/uni-semi-sup-depth.tex <==


\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{rlll}
\toprule
Method & \multicolumn{1}{l}{0.1\% (49)} & \multicolumn{1}{l}{0.2\% (98)} & \multicolumn{1}{l}{1\% (491)} \\ \midrule
Uni-modal (sup-only) & 34.05 & 35.24 & 44.78 \\
Uni-modal + MT \cite{mt}& 33.46 & 37.57 & \underline{46.25} \\ 
Uni-modal + CPS-Seg\footnoteref{note:cps-seg} \cite{chen2021-CPS} & 33.56 & 36.71 & 45.71 \\ \midrule
% Segformer & 35.43 & 39.45 & 46.45 \\
% Segformer + MT & 36.59 & 41.5 & 47.04 \\ \midrule
% LF (RGB) & 32.58 & 33.66 & 33.51 \\
% LF + MT (RGB)& 32.37 & 33.99 & 33.65 \\ \midrule
Ours & \textbf{39.93} \add{5.88}& \textbf{42.70} \add{5.13}& \textbf{46.79} \add{0.54}\\ \bottomrule
\end{tabular}
}
\caption{\small{\textbf{Multi-modal training benefits the uni-modal segmentation results.} 
Performance with \textit{depth} input of our proposed LF+M3L method as compared to uni-modal Segformer \cite{segformer} supervised only 
and semi-supervised (MT, CPS) models on Stanford Indoor dataset \cite{stanfordindoor}}}
\label{tab:uni-semi-sup-depth}
\end{table}

==> tables/uni-semi-sup-rgb.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{rlll}
\toprule
Method & \multicolumn{1}{l}{0.1\% (49)} & \multicolumn{1}{l}{0.2\% (98)} & \multicolumn{1}{l}{1\% (491)} \\ \midrule
Uni-modal (sup-only) & 35.43 & 39.45 & 46.45 \\
Uni-modal + MT \cite{mt}& 36.59 & 41.50 & 47.04 \\
Uni-modal + CPS-Seg\footnoteref{note:cps-seg} \cite{chen2021-CPS}& 37.09 & 42.75 & 46.37 \\ \midrule
% Segformer & 35.43 & 39.45 & 46.45 \\
% Segformer + MT & 36.59 & 41.5 & 47.04 \\ \midrule
% LF (RGB) & 32.58 & 33.66 & 33.51 \\
% LF + MT (RGB)& 32.37 & 33.99 & 33.65 \\ \midrule
Ours & \textbf{40.05} \add{2.96}& \textbf{44.62} \add{1.87}& \textbf{49.28} \add{2.24}\\ \bottomrule
\end{tabular}
}
\caption{\small{\textbf{Multi-modal training benefits the uni-modal segmentation results.} 
Performance with \textit{RGB} input of our proposed LF+M3L method as compared to uni-modal Segformer \cite{segformer} supervised only 
and semi-supervised (MT, CPS) models on Stanford Indoor dataset \cite{stanfordindoor}}}
\label{tab:uni-semi-sup-rgb}
\end{table}

% \begin{table*}[t]
% \centering
% \resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{rccc|ccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{RGB Uni-modal} & \multicolumn{3}{c}{Depth Uni-modal} \\
% \multicolumn{1}{c}{} & 0.1\% (49) & 0.2\% (98) & 1\% (491) & 0.1\% (49) & 0.2\% (98) & 1\%(491) \\ \midrule
% Uni-modal (sup-only) & 35.43 & 39.45 & 46.45 & 34.05 & 35.24 & 44.78 \\
% Uni-modal + MT \cite{mt} & 36.59 & 41.50 & 47.04 & 33.46 & 37.57 & \underline{46.25} \\
% Uni-modal + CPS-Seg\footnoteref{note:cps-seg} \cite{chen2021-CPS} & 37.09 & 42.75 & 46.37 & 33.56 & 36.71 & 45.71 \\ \midrule
% Ours & \textbf{40.05} \add{2.96}& \textbf{44.62} \add{1.87}& \textbf{49.28} \add{2.24} & \textbf{39.93} \add{5.88} & \textbf{42.70} \add{5.13} & \textbf{46.79} \add{0.54} \\ \bottomrule
% \end{tabular}
% }
% \caption{\small{\textbf{Multi-modal training benefits the uni-modal segmentation results.} 
% Performance with \textit{RGB}-only and \textit{depth}-only input  of our proposed LF+M3L method as compared to uni-modal Segformer \cite{segformer} supervised only 
% and semi-supervised (MT, CPS) models on Stanford Indoor dataset \cite{stanfordindoor}}}
% \label{tab:uni-semi-sup-rgb}
% \end{table*}


